First Search for Axion-Like Particles in a Storage Ring Using a Polarized Deuteron Beam

Based on the notion that the local dark-matter field of axions or axion-like particles (ALPs) in our Galaxy induces oscillating couplings to the spins of nucleons and nuclei (via the electric dipole moment of the latter and/or the paramagnetic axion-wind effect), we establish the feasibility of a new method to search for ALPs in storage rings. Based on previous work that allows us to maintain the in-plane polarization of a stored deuteron beam for a few hundred seconds, we performed a first proof-of-principle experiment at the Cooler Synchrotron COSY to scan momenta near 970 MeV/c. This entailed a scan of the spin precession frequency. At resonance between the spin precession frequency of deuterons and the ALP-induced EDM oscillation frequency there will be an accumulation of the polarization component out of the ring plane. Since the axion frequency is unknown, the momentum of the beam and consequently the spin precession frequency were ramped to search for a vertical polarization change that would occur when the resonance is crossed. At COSY, four beam bunches with different polarization directions were used to make sure that no resonance was missed because of the unknown relative phase between the polarization precession and the axion/ALP field. A frequency window of 1.5-kHz width around the spin precession frequency of 121 kHz was scanned. We describe the experimental procedure and a test of the methodology with the help of a radiofrequency Wien filter located on the COSY ring. No ALP resonance was observed. As a consequence an upper limit of the oscillating EDM component of the deuteron as well as its axion coupling constants are provided.

==> authorlist.tex <==
\author{S.\,Karanth}
\email{swathi.karanth@doctoral.uj.edu.pl}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{E.J.\,Stephenson}
\email{stephene@iu.edu}
\affiliation{Indiana University, Department of Physics, Bloomington, IN 47405, USA}

\author{S.P.\,Chang}
\affiliation{Department of Physics, KAIST, Daejon 34141, Republic of Korea}
\affiliation{Center for Axion and Precision Physics Research, IBS, Daejon 34141, Republic of Korea}

\author{V.\,Hejny}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{J.\,Pretz}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

\author{Y.\,Semertzidis}
\affiliation{Department of Physics, KAIST, Daejon 34141, Republic of Korea}
\affiliation{Center for Axion and Precision Physics Research, IBS, Daejon 34141, Republic of Korea}

\author{A.\,Wirzba}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{Institute for Advanced Simulation, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.\,Wro\'{n}ska}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{F.\,Abusaif}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}

\author{A.\,Aksentev}
%\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{Institute for Nuclear Research, Russian Academy of Sciences, 117312 Moscow, Russia}

\author{B.\,Alberdi}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}



\author{A.\,Aggarwal}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{A.\,Andres}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}


\author{L.\,Barion}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{I.\,Bekman}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}

\affiliation{{\rm now at:} Zentralinstitut f\"ur Engineering, Elektronik und Analytik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}



\author{M.\,Bey{\ss}}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}

\author{C.\,B\"ohme}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{B.\,Breitkreutz}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich,  52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}


\author{C.\,von Byern} %former Kaeseberg
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}


\author{N.\,Canale}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{G.\,Ciullo}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{S.\,Dymov}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{N.-O.\,Fr\"ohlich}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at} 
DESY, Deutsches Elektronen-Synchrotron, 22607 Hamburg, Germany}

\author{R.\,Gebel}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

%\author{M.\,Gaisser}
%\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\author{K.\,Grigoryev}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{D.\,Grzonka}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{J.\,Hetzel}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}


\author{O.\,Javakhishvili}
\affiliation{Department of Electrical and Computer Engineering, Agricultural University of Georgia, 0159 Tbilisi, Georgia}

\author{H.\,Jeong}
\affiliation{Center for Axion and Precision Physics Research, IBS, Daejon 34141, Republic of Korea}

\author{A.\,Kacharava}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{V.\,Kamerdzhiev}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}


\author{I.\,Keshelashvili}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{A.\,Kononov}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}\

\author{K.\,Laihem}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{A.\,Lehrach}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

\author{P.\,Lenisa}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{N.\,Lomidze}
\affiliation{High Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{B.\,Lorentz}
\affiliation{GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{A.\,Magiera}
\affiliation{Marian Smoluchowski Institute of Physics, Jagiellonian University, 30348 Cracow, Poland}

\author{D.\,Mchedlishvili}
\affiliation{High Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{F.\,Müller}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{A.\,Nass}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{N.N.\,Nikolaev}
\affiliation{L.D. Landau Institute for Theoretical Physics, 142432 Chernogolovka, Russia}

\author{S.\,Park}
\affiliation{Center for Axion and Precision Physics Research, IBS, Daejon 34141, Republic of Korea}

\author{A.\,Pesce}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{V.\,Poncza}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{D.\,Prasuhn}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}


\author{F.\,Rathmann}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{S.\,Siddique}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{A.\,Saleev}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{N.\,Shurkhno}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

%\author{Yu.\,Senichev}
%\affiliation{Institute for Nuclear Research, Russian Academy of Sciences, 117312 Moscow, Russia}

\author{D.\,Shergelashvili}
\affiliation{High Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{V.\,Shmakova}
\affiliation{University of Ferrara and Istituto Nazionale di Fisica Nucleare, 44100 Ferrara, Italy}

\author{J.\,Slim}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{H.\,Soltner}
\affiliation{Zentralinstitut f\"ur Engineering, Elektronik und Analytik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{R.\,Stassen}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}


\author{H.\,Ströher}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{JARA--FAME (Forces and Matter Experiments), Forschungszentrum J\"ulich and RWTH Aachen University, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}


\author{M.\,Tabidze}
\affiliation{High Energy Physics Institute, Tbilisi State University, 0186 Tbilisi, Georgia}

\author{G.\,Tagliente}
\affiliation{Istituto Nazionale di Fisica Nucleare sez.\ Bari, 70125 Bari, Italy}
  
\author{Y.\,Valdau}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

\author{M.\,Vitz}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}


\author{T.\,Wagner}
\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}
\affiliation{III.\ Physikalisches Institut B, RWTH Aachen University, 52056 Aachen, Germany}

\affiliation{{\rm now at:} 
GSI Helmholtzzentrum für Schwerionenforschung, 64291 Darmstadt, Germany}

%\author{C.\,Weidemann}
%\affiliation{Institut f\"ur Kernphysik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

\author{P.\,W\"ustner}
\affiliation{Zentralinstitut f\"ur Engineering, Elektronik und Analytik, Forschungszentrum J\"ulich, 52425 J\"ulich, Germany}

%\author{M.\,\.{Z}urek}
%\affiliation{Lawrence Berkeley National Laboratory, Berkeley, California 94720, USA}
%\affiliation{Argonne National Laboratory, Lemont, Illinois 60439, USA - current (2022)}


\collaboration{JEDI Collaboration}
\noaffiliation

